Open-Set Semi-Supervised Object Detection

Recent developments for Semi-Supervised Object Detection (SSOD) have shown the promise of leveraging unlabeled data to improve an object detector. However, thus far these methods have assumed that the unlabeled data does not contain out-of-distribution (OOD) classes, which is unrealistic with larger-scale unlabeled datasets. In this paper, we consider a more practical yet challenging problem, Open-Set Semi-Supervised Object Detection (OSSOD). We first find the existing SSOD method obtains a lower performance gain in open-set conditions, and this is caused by the semantic expansion, where the distracting OOD objects are mispredicted as in-distribution pseudo-labels for the semi-supervised training. To address this problem, we consider online and offline OOD detection modules, which are integrated with SSOD methods. With the extensive studies, we found that leveraging an offline OOD detector based on a self-supervised vision transformer performs favorably against online OOD detectors due to its robustness to the interference of pseudo-labeling. In the experiment, our proposed framework effectively addresses the semantic expansion issue and shows consistent improvements on many OSSOD benchmarks, including large-scale COCO-OpenImages. We also verify the effectiveness of our framework under different OSSOD conditions, including varying numbers of in-distribution classes, different degrees of supervision, and different combinations of unlabeled sets.

==> figure/boundary_wise_reg_conf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figure/pic/reg_conf.pdf}
    \caption{Comparison between the boundary-level and the box-level pseudo-labels. We aim to only enforce the unsupervised regression loss on the accurately predicted pseudo-boundaries (color in red).}
    \label{fig:boundary_wise_regconf}
\end{figure}


==> figure/pseudo_anchor_free.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figure/pic/pseudo_anchor_free.pdf}
    \caption{Illustration of the center-sampling and localization-weighted classification labels, which is generated from the pseudo-labels.}
    \label{fig:pseudo_anchor_free}
\end{figure}

% \begin{figure}[t]
% \centering
% \subfloat[Heuristic-Based Level Assignment]{%
%   \includegraphics[width=.45\linewidth]{figure/pic/pseudo_anchor_free.pdf}%
%   \label{fig:heuristic}%
% }\qquad
% \subfloat[Training with All-Level Features]{%
%   \includegraphics[width=.45\linewidth]{figures/pic/all_level.png}%
%   \label{fig:all_level}%
% }
% \caption{Comparison between heuristic-based level assignment in Faster R-CNN and our proposed training with All-Level Features}
% \label{fig:fpn}
% \end{figure}

==> figure/pseudo_label_weakness.tex <==

\begin{figure}[t]
\centering
\subfloat[Unreliable label assignment]{%
  \includegraphics[width=.45\linewidth]{figure/pic/pseudo_anchor_free.pdf}%
  \label{fig:label_assignment}%
}\qquad
\subfloat[Box-level vs. Boundary-level pseudo-label for regression]{%
  \includegraphics[width=.45\linewidth]{figure/pic/reg_conf.pdf}%
  \label{fig:reg_label_level}%
}
\caption{(a) Label assignments of some existing anchor-free models~\cite{tian2019fcos,li2020generalized,li2020gflv2} are less robust to the localization noise (\textit{e.g.,} box center shift) in pseudo-boxes used in semi-supervised training. (b) Rather than box-level pseudo-label used in the existing SS-OD works, we aim to select the precisely predicted boundary and use boundary-level pseudo-labels for improving the bounding box regression branch.
\yc{Need to make a new figures to convey two major messages: anchor-free detectors and regression loss}
} 
\label{fig:fpn}
\end{figure}

==> figure/unreliable_label.tex <==

\begin{figure}[t]
\centering
\subfloat[Label assignments]{%
  \includegraphics[width=.5\linewidth]{figure/pic/pseudo_anchor_free.pdf}%
  \label{fig:label_assignment_vis}%
}\qquad
\subfloat[mAP comparison]{%
  \includegraphics[width=.22\linewidth]{figure/pic/label_assignment.pdf}%
  \label{fig:label_assignment_results}%
}
\caption{
(a) Existing techniques for improving fully-supervised anchor-free detectors such as Center-sampling~\cite{tian2019fcos} and localization-based soft classification labels~\cite{li2020generalized} are less robust to the localization noise (\textit{e.g.,} box center shifted) in pseudo-boxes used in semi-supervised training, and the pixel-wise recall and precision of these two techniques are lower than the standard label assignment. Thus, (b) our empirical evaluation shows that the standard label assignment leads to a better result.
% \zk{It's really hard to interpret these methods on left without knowing the methods. This might be a good candidate for moving to appendix}\yc{Add recall/precision of pixels}
} 
\label{fig:fpn}
% \vspace{-5mm}
\end{figure}

==> impact.tex <==
% \section{Broader Impact}

% Our work discusses a fundamental problem in deep learning: data imbalance. Data imbalance can be safety-critical in many applications such as self-driving. Our approach allows an algorithm to give more attention to pedestrians and small obstacles. Additionally, our unified algorithm aims to provide stable performance under severe visual degradation which is also critical for safty considerations.   

==> table/analysis-breakdown-all.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Average precision (AP) breakdown of the model with and without our \proposedregmethod.}
\vspace{1mm}
\label{table:ap_breakdown}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccc}
\toprule
        %   & \multicolumn{5}{c}{\textbf{Anchor-free detectors} on COCO-standard}  \\ \cline{2-6}
                           &  AP50 & AP55  & AP60  & AP65  & AP 70  & AP75& AP80 & AP85 & AP90 & AP95\\ \hline
No regression    & 31.53 & 29.71 & 27.34 & 24.64 &  21.38 & 17.55 & 13.27 & 8.33  & 3.45 & 0.35  \\ 
Confidence thresholding    & 32.59 & 30.78 & 28.59 & 26.19 &  23.05 & 19.64 & 15.61 & 10.47 & 5.06 & 0.58 \\ \hline
\proposedregmethod\    & 32.59 & 30.78 & 28.59 & 26.19 &  23.05 & 19.64 & 15.61 & 10.47 & 5.06 & 0.58 \\ \hline
% Absolute Improvement (mAP) & +1.06 & +1.07 & +1.25 & +1.56 &  +1.67 & +2.09 & +2.34 & +2.14 & +1.61 & +0.23 \\ 
Relative Improvement (\%)  & \textcolor{myblue}{+3.36} & \textcolor{myblue}{+3.60} & \textcolor{myblue}{+4.57} & \textcolor{myblue}{+6.29} &  \textcolor{myblue}{+7.81} & \textcolor{myblue}{+11.91} & \textcolor{myblue}{+17.63} & \textcolor{myblue}{+25.69} & \textcolor{myblue}{+46.67} & \textcolor{myblue}{+65.71} \\ 
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/analysis-unsup_reg.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{Ablation study of unsupervised regression loss.}
% % We ablate different unsupervised regression loss on our anchor-free model, and our~\proposedregmethod\ can perform favorably against the existing unsupervised regression loss.}
% % \yc{I didn't change this, as the ablation of modifications to anchor-free models are verified in Figure~\ref{fig:centerness_bias} and \ref{fig:label_assignment_results}}
% \vspace{1mm}
% \label{table:ablate_ureg}
% \resizebox{0.5\linewidth}{!}{%
% \begin{tabular}{cccc}
% \toprule
%           & \multicolumn{3}{c}{COCO-standard 1\% }  \\ \cline{2-4}
% \multirow{2}{*}{Methods}      & \proposedregmethod &  \multirow{2}{*}{Confidence thresholding}    & \multirow{2}{*}{No regression}   \\ 
%           & (Ours) &   &       \\ \hline
%             &  19.28            &     18.27          &   17.79   \\ 
% \bottomrule
% \end{tabular}
% }
% \vspace{-3mm}
% \end{table}




% Vertical version
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{Ablation study of unsupervised regression loss.}
% % We ablate different unsupervised regression loss on our anchor-free model, and our~\proposedregmethod\ can perform favorably against the existing unsupervised regression loss.}
% % \yc{I didn't change this, as the ablation of modifications to anchor-free models are verified in Figure~\ref{fig:centerness_bias} and \ref{fig:label_assignment_results}}
% \label{table:ablate_ureg}
% \begin{tabular}{c|c}
% \toprule
%                   & mAP   \\\hline
% No Regression      & 17.79 \\
% Conf. Thresholding & 18.27 \\
% ~\proposedregmethod   (Ours) & 19.56\\
% \bottomrule
% \end{tabular}
% \vspace{-3mm}
% \end{table}


\begin{table*}[!t]
\begin{minipage}[t]{0.68\textwidth}
\captionof{table}{ {Results of the {anchor-free model (FCOS)} on \textit{VOC}}.}  
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccl}
\Xhline{2\arrayrulewidth}
          & \multicolumn{4}{c}{\textbf{Anchor-free detectors} on VOC}  \\ \cline{2-5}
 & Models & Labeled & Unlabeled  & \multicolumn{1}{c}{$AP_{50:95}$} \\ \hline
 Supervised& \scriptsize{FCOS-R50}  & VOC07 & None & 41.53  \\\hline
% Supervised (from STAC)& \scriptsize{ResNet50-FPN}  & VOC07 & None & 42.60  \\ 
% CSD & \scriptsize{ResNet101-R-FCN}  & \multirow{3}{*}{VOC07} & \multirow{3}{*}{VOC12}   & -   \\ 
STAC~\cite{sohn2020simple} & \scriptsize{FCOS-R50} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{VOC12}  & 44.47 \scriptsize{\textcolor{myblue}{(+2.94)}}  \\
Unbiased Teacher~\cite{liu2021unbiased} & \scriptsize{FCOS-R50} &   &   & 49.50 \scriptsize{\textcolor{myblue}{(+7.97)}}  \\
Ours & \scriptsize{FCOS-R50} & &  & \textbf{51.47 \scriptsize{\textcolor{myblue}{(+9.94)}}}\\ \hline
% CSD & \scriptsize{ResNet101-R-FCN} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VOC12\\ +\\ \textit{COCO20cls}\end{tabular}}  & -   \\ 
STAC~\cite{sohn2020simple} & \scriptsize{FCOS-R50} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VOC12 \\+\\ \textit{COCO20cls}\end{tabular}}  & 44.89 \scriptsize{\textcolor{myblue}{(+3.36)}}  \\
Unbiased Teacher~\cite{liu2021unbiased} & \scriptsize{FCOS-R50} &  &  & 51.15 \scriptsize{\textcolor{myblue}{(+9.62)}}  \\
Ours & \scriptsize{FCOS-R50}  & &   & \textbf{52.95 \scriptsize{\textcolor{myblue}{(+11.42)}}} \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
% We observe that the Baseline gets relatively higher as the domain difference gets larger.
\label{table:voc}
\end{minipage}
\hfill
\begin{minipage}[t]{0.3\textwidth}
\captionof{table}{Ablation study of unsupervised regression loss. All methods use FCOS in COCO-standard 1$\%$.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc}
\toprule
                  & mAP   \\\hline
No Regression      & 17.79 \\
Conf. Thresholding & 18.27 \\
~\proposedregmethod\  (Ours)               & \textbf{19.56}\\
\bottomrule
\end{tabular}
}
\label{table:ablate_ureg}
\end{minipage}
\end{table*}

==> table/analysis_breakdown.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Average precision (AP) breakdown of the model with and without our \proposedregmethod.}
\vspace{1mm}
\label{table:ap_breakdown}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccc}
\toprule
        %   & \multicolumn{5}{c}{\textbf{Anchor-free detectors} on COCO-standard}  \\ \cline{2-6}
                           &  AP50 & AP55  & AP60  & AP65  & AP 70  & AP75& AP80 & AP85 & AP90 & AP95\\ \hline
w/o \proposedregmethod\    & 31.53 & 29.71 & 27.34 & 24.64 &  21.38 & 17.55 & 13.27 & 8.33  & 3.45 & 0.35  \\ 
w/  \proposedregmethod\    & 32.59 & 30.78 & 28.59 & 26.19 &  23.05 & 19.64 & 15.61 & 10.47 & 5.06 & 0.58 \\ \hline
% Absolute Improvement (mAP) & +1.06 & +1.07 & +1.25 & +1.56 &  +1.67 & +2.09 & +2.34 & +2.14 & +1.61 & +0.23 \\ 
Relative Improvement (\%)  & \textcolor{myblue}{+3.36} & \textcolor{myblue}{+3.60} & \textcolor{myblue}{+4.57} & \textcolor{myblue}{+6.29} &  \textcolor{myblue}{+7.81} & \textcolor{myblue}{+11.91} & \textcolor{myblue}{+17.63} & \textcolor{myblue}{+25.69} & \textcolor{myblue}{+46.67} & \textcolor{myblue}{+65.71} \\ 
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}


==> table/anchor2free.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
    \textbf{Adaption of Unbiased Teacher~\cite{liu2021unbiased} to anchor-free model}. The performance is degraded when applying Unbiased Teacher on the anchor-free model (FCOS). 
    % \zk{ (FCOS?)}\kevin{We should also have a column to show supervised baseline comparison between Faster-RCNN and FCOS with 100\% COCO data. This is to show that Faster-RCNN and FCOS should be comparable to each other in the supervised setting.}\yc{Added.}
    }
    %Note that we use ResNet50 as the feature backbone for both methods.}
\vspace{1mm}
\label{table:anchor2free}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccccc||c}
\toprule
           & &\multicolumn{5}{c||}{COCO-standard}  & Upperbound \\ \cline{3-8}
    Methods       & Models &\multicolumn{1}{c}{0.5\%}
  &\multicolumn{1}{c}{1\%}     & \multicolumn{1}{c}{2\%}    & \multicolumn{1}{c}{5\%}    & \multicolumn{1}{c||}{10\%}   &  100\% \\ \hline
% Supervised & Faster-RCNN &  6.83 &  9.05       &    12.70   &    18.47  &    23.86           \\ 
% Supervised & FCOS &  6.01 &  8.56       &    12.37   &    17.07  &    21.36           \\ \hline
Unbiased Teacher~\cite{liu2021unbiased} &  Faster-RCNN  & 14.36 &   18.33 & 22.23 &  26.65 &  29.56 & 37.63 \\ 
Unbiased Teacher~\cite{liu2021unbiased} &  FCOS         & 10.27  \scriptsize{\textcolor{red}{(-4.09)}}&   14.61 \scriptsize{\textcolor{red}{(-3.72)}} & 18.70 \scriptsize{\textcolor{red}{(-3.53)}} &  23.99 \scriptsize{\textcolor{red}{(-2.66)}} & 28.18 \scriptsize{\textcolor{red}{(-1.38)}} & 37.10\\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}



% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{
%     \textbf{Adaption of Unbiased Teacher~\cite{liu2021unbiased} to anchor-free model}, and performance is degraded when Unbiased Teacher is adapted to anchor-free model. Note that we use ResNet50 as the feature backbone for all methods.}
% \vspace{1mm}
% \label{table:anchor2free}
% % \resizebox{\linewidth}{!}{%
% \begin{tabular}{lll}
% \toprule
%           &\multicolumn{2}{c}{COCO-standard $0.05\%$}  \\ \hline
%     Methods       & \multicolumn{1}{c}{Faster-RCNN}  &\multicolumn{1}{c}{FCOS}        \\ \hline
% % Supervised & Faster-RCNN &  6.83 &  9.05       &    12.70   &    18.47  &    23.86           \\ 
% % Supervised & FCOS &  6.01 &  8.56       &    12.37   &    17.07  &    21.36           \\ \hline
% Supervised only &    6.83  &  6.01  \\ 
% Unbiased Teacher~\cite{liu2021unbiased} &   14.36 &   9.75 \\ 
% \bottomrule
% \end{tabular}
% %}
% \vspace{-3mm}
% \end{table}


==> table/augment.tex <==
\begin{table}[ht]
    \centering
    \caption{
Detail of data augmentations. Probability in the table indicates the probability of applying the corresponding image process.}
    \label{table:data_aug_parameter}
    \vspace{3mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccl}
\toprule\toprule
\multicolumn{4}{c}{\textbf{Weak Augmentation}}\\
\midrule
Process& Probability & Parameters& \multicolumn{1}{c}{Descriptions}\\
\midrule
Horizontal Flip & 0.5& -& \multicolumn{1}{c}{None}\\ \midrule \midrule
\multicolumn{4}{c}{\textbf{Strong Augmentation}}\\ \midrule
Process         & Probability & Parameters& \multicolumn{1}{c}{Descriptions}\\\midrule
Color Jittering & 0.8                     & \begin{tabular}[c]{@{}c@{}}(brightness, contrast, saturation, hue)\\ = (0.4, 0.4, 0.4, 0.1)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Brightness factor is chosen uniformly from {[}0.6, 1.4{]},\\ contrast factor is chosen uniformly from {[}0.6, 1.4{]},\\ saturation factor is chosen uniformly from {[}0.6, 1.4{]},\\ and hue value is chosen uniformly from {[}-0.1, 0.1{]}.\end{tabular} \\ \midrule
Grayscale       & 0.2                     & None                                                                                                       & \multicolumn{1}{c}{None}                                                                                                                                                                                                                                                                                    \\  \midrule
GaussianBlur    & 0.5                     & (sigma\_x, sigma\_y) = (0.1, 2.0)                                                                        & Gaussian filter with $\sigma_x=0.1$ and $\sigma_y=2.0$ is applied.                                                                                                                                                                                                                   \\ \midrule
CutoutPattern1  & 0.7                     & scale=(0.05, 0.2),  ratio=(0.3, 3.3)                                                                     & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels. We refer the detail in~\cite{zhong2017random}.\end{tabular}                                                                                                                                             \\ \midrule
CutoutPattern2  & 0.5                     & scale=(0.02, 0.2), ratio=(0.1, 6)                                                                        & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels. We refer the detail in~\cite{zhong2017random}.\end{tabular}                                                                                                                                             \\ \midrule
CutoutPattern3  & 0.3                     & scale=(0.02, 0.2), ratio=(0.05, 8)                                                                       & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels. We refer the detail in~\cite{zhong2017random}.\end{tabular}
\\
\bottomrule\bottomrule
\end{tabular}}
\end{table}


==> table/coco-add-sota.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
% \kevin{This table is not mentioned in the text. Also, why do we want to have a separate table for COCO-additional?}
% \kevin{Do we have experimental results for UT + OF-ViT?}
Comparison to other SSOD methods in COCO-additional. The supervised baseline is trained with same batch size and iterations. The result of MOCOv2 is reported by Humble Teacher~\cite{tang2021humble}, and the supervised baseline is trained with same batch size and training iterations.
}
% \vspace{-3mm}
\label{table:cocoadd_sota}
\resizebox{0.3\linewidth}{!}{
\begin{tabular}{cc}
\toprule
                                              & mAP   \\ 
                                              \midrule
% \specialrule{1pt}{1pt}{1pt}
Supervised                                                     & 40.90 \\ \midrule
Proposal Learning~\cite{tang2020proposal}                      & 38.40 \\
CSD~\cite{jeong2019consistency}                                & 38.82 \\
STAC~\cite{sohn2020simple}                                     & 39.21 \\
Instant-Teaching~\cite{zhou2021instant}                        & 40.20 \\
% MOCOv2 + MS-COCO unlabel~\cite{tang2021humble}                 & 35.29 \\
% MOCOv2 + ImageNet-1M~\cite{tang2021humble}                     & 40.80 \\
MOCOv2 + Instagram-1B~\cite{tang2021humble}                    & 41.10 \\
Humble Teacher~\cite{tang2021humble}                           & 42.37 \\
SoftTeacher\tablefootnote{The performance of SoftTeacher is obtained from their GitHub [\href{https://github.com/microsoft/SoftTeacher}{link}].}~\cite{xu2021end}                                   & 44.05 \\
Unbiased Teacher*~\cite{liu2021unbiased}                       & 44.06 \\ 
Unbiased Teacher* + OF-DINO                                    & \textbf{45.14} \\ \midrule
Unbiased Teacher* + OF-ViT                                   & 45.16 \\ 
\bottomrule
\end{tabular}
}
\vspace{-6mm}
\end{table}


==> table/coco-add.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
\kevin{There is no comparison with the other SoTAs?}\zk{This seems the same as Table 8? Maybe we can mention full results are there? It's generally not clear why this table is here; why don't we just use Table 8 to show these things (adding supervised baseline and iterations, etc.?). Otherwise mention here the point of the table (COCO-additional is not the point). }
\kevin{Why do we show number of training iterations? We did not discuss this in the paper.}
Experimental results of \textbf{COCO-additional}.
UT* is the Unbiased Teacher~\cite{liu2021unbiased} trained along with the data augmentation used in SoftTeacher~\cite{xu2021end}.
}
\vspace{1mm}
\label{table:coco-add}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{ccc}
\toprule
           &    Training iterations                               & mAP   \\ \specialrule{1pt}{1pt}{1pt}
           & 90k                                                    & 37.90 \\
Supervised & 270k                                                    & 40.20 \\
           & 720k                                                    & 40.90 \\ \midrule
UT*~\cite{liu2021unbiased}& 720k                        & 44.06 \\ 
UT* + OF-DINO  &    720k                             & \textbf{45.14} \\
UT* + OF-ViT   &    720k                             & \textbf{45.15} \\ \bottomrule
\end{tabular}
}
% \vspace{-3mm}
\end{table}


==> table/coco-full.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Experimental results of COCO-GOI.}
\vspace{1mm}
\label{table:ap_breakdown_all}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{cc}
\toprule
                                                                   & mAP   \\ \specialrule{1pt}{1pt}{1pt}
Supervised (1x)                                                    & 37.90 \\
Supervised (3x)                                                    & 40.20 \\
Supervised (8x)                                                    & 40.90 \\ 
Unbiased Teacher~\cite{liu2021unbiased}                            & 43.70 \\ \midrule
Unbiased Teacher + OOD (DINO)                                      & 44.91 \\
Unbiased Teacher + OOD (ViT)                                       & 45.06 \\ \bottomrule
\end{tabular}
% }
% \vspace{-3mm}
\end{table}


==> table/coco-open-source.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Experimental results on varying types and numbers of unlabeled data in the task of \textbf{COCO-Open 40-4k}. Note that OF represents OOD filtering.}
\vspace{1mm}
\label{table:data_source}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
                                    % & \multicolumn{3}{c}{COCO 40 - 4k}                      \\ \cmidrule{2-4}
Unlabeled Data Type                 & \textcolor{red}{ID}  & \textcolor{red}{ID}+\textcolor{myblue}{Mix}   & \textcolor{red}{ID}+\textcolor{myblue}{Mix}+\textcolor{orange}{OOD}  \\ 
Amount of Unlabeled Data               & 32, 091 & 94,144 & 113,266 \\ \specialrule{1pt}{1pt}{1pt}
Labeled Only                        & 16.07   & 16.07            & 16.07                          \\ 
Unbiased Teacher~\cite{liu2021unbiased}                    & 22.10   & 20.04            & 19.93                     \\ \midrule
Unbiased Teacher~\cite{liu2021unbiased}  + OF-DINO       & 22.40   & 23.60            & 23.31                     \\ 
Unbiased Teacher~\cite{liu2021unbiased}  + OF-ViT      & 23.90   & 25.63            & 25.32                     \\ 
% Upper-reference: All inlier objects & 34.36   & 34.36            & 34.36                     \\ 
\bottomrule
\end{tabular}
}
% \vspace{-3mm}
\end{table}


==> table/coco_additioal_anchor_free.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{\textcolor{black}{
    {Experimental results of the anchor-free model (FCOS-ResNet50) on \textit{COCO-additional}}.
    Note that 1x represents 90K training iterations, and $N$x represents $N\times$90K training iterations. 
    % \zk{Should we add amount of improvement?}
    % \kevin{Is Ours here anchor-free or anchor-based?}\yc{All methods in this table are anchor-free detectors}
    }
    }
\label{table:mscoco-add}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
          & \multicolumn{6}{c}{\textbf{Anchor-free detectors} on COCO-additional}  \\ \cline{2-7}
          & Supervised (1x) & Supervised (3x) & CSD (3x)   & STAC (3x)  &Unbiased Teacher (3x)  & Ours (3x)   \\ \hline
$AP^{50:95}$&  37.10 & 37.29 & 36.70 \scriptsize{\textcolor{red}{(-0.59)}}  &   38.06 \scriptsize{\textcolor{myblue}{(+0.77)}}   & 39.84 \scriptsize{\textcolor{myblue}{(+2.55)}} & \textbf{40.97 \scriptsize{\textcolor{myblue}{(+3.68)}}}    \\ 

\bottomrule
\end{tabular}}
\end{table*}


==> table/coco_standard_anchor_free.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
    {Experimental results of the anchor-free model (FCOS-ResNet50) on \textit{COCO-standard}}. * We used their implementation and adapt to FCOS-ResNet50. 
    We randomly sample labeled data and run each method $5$ times, and we report the mean and standard deviation for each result.
    % \zk{For STAC you didn't use their implementation and adapt to FCOS (no star)? How did you get anchor-free numbers then? Did your implementation of STAC under anchor-based method reproduce their results? Might need to mention this} \yc{Added star for STAC}
    % Note that instant-teaching~\cite{zhou2021instant} and Humble Teacher~\cite{tang2021humble} share the similar prope
    }
\vspace{1mm}
\label{table:mscoco_standard_anchor_free}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llllll}
\toprule
           & \multicolumn{5}{c}{\textbf{Anchor-free detectors} on COCO-standard}  \\ \cline{2-6}
           & \multicolumn{1}{c}{0.5\%}
  &\multicolumn{1}{c}{1\%}     & \multicolumn{1}{c}{2\%}    & \multicolumn{1}{c}{5\%}    & \multicolumn{1}{c}{10\%}     \\ \hline
Supervised&  5.42 $\pm$ 0.01 &  8.43 $\pm$ 0.03    &    11.97 $\pm$ 0.03 &    17.01 $\pm$  0.01 &  20.98  $\pm$ 0.01        \\ \hline
CSD~\cite{jeong2019consistency}*     & 5.76 $\pm$ 0.55  \scriptsize{\textcolor{myblue}{(+0.34)}} & 9.23 $\pm$ 0.08  \scriptsize{\textcolor{myblue}{(+0.80)}} & 12.53 $\pm$ 0.04  \scriptsize{\textcolor{myblue}{(+0.56)}} & 18.09 $\pm$ 0.08 \scriptsize{\textcolor{myblue}{(+1.08)}} & 22.06 $\pm$ 0.01 \scriptsize{\textcolor{myblue}{(+1.08)}} \\ 
% CSD~\cite{jeong2019consistency}     & run &   run & run &  run &  run \\ 
STAC~\cite{sohn2020simple}*     & 8.79 $\pm$ 0.12 \scriptsize{\textcolor{myblue}{(+3.37)}} &   11.97 $\pm$ 0.12 \scriptsize{\textcolor{myblue}{(+3.54)}} & 15.50 $\pm$ 0.16 \scriptsize{\textcolor{myblue}{(+3.53)}}&  20.36 $\pm$ 0.05 \scriptsize{\textcolor{myblue}{(+3.35)}} &  24.31 $\pm$ 0.02 \scriptsize{\textcolor{myblue}{(+3.33)}}\\ 
Unbiased Teacher~\cite{liu2021unbiased}*     & 10.27  $\pm$ 0.13 \scriptsize{\textcolor{myblue}{(+4.85)}} &  14.61 $\pm$ 0.10 \scriptsize{\textcolor{myblue}{(+6.18)}} & 18.70 $\pm$ 0.21 \scriptsize{\textcolor{myblue}{(+6.73)}} &  23.99 $\pm$ 0.12 \scriptsize{\textcolor{myblue}{(+6.98)}} &  28.18 $\pm$ 0.01 \scriptsize{\textcolor{myblue}{(+7.20)}} \\ 
\textbf{Ours}      & \textbf{14.28 $\pm$ 0.23 \scriptsize{\textcolor{myblue}{(+8.86)}}}& \textbf{19.56 $\pm$ 0.24  \scriptsize{\textcolor{myblue}{(+11.13)}} }& \textbf{22.88 $\pm$ 0.06 \scriptsize{\textcolor{myblue}{(+10.91)}}} &  \textbf{26.84 $\pm$ 0.03 \scriptsize{\textcolor{myblue}{(+9.83)}}}  &  \textbf{29.61 $\pm$ 0.02 \scriptsize{\textcolor{myblue}{(+8.63)}}} \\
\bottomrule
\end{tabular}
}
% \vspace{-3mm}
\end{table*}


==> table/rebuttal/openmatch.tex <==
\begin{table}[h]
\centering
\vspace{-3mm}
\renewcommand{\arraystretch}{1.3}
\caption{Comparison to OpenMatch
(Saito et el., \href{https://papers.nips.cc/paper/2021/hash/da11e8cd1811acb79ccf0fd62cd58f86-Abstract.html}{NeurIPS'21}), the SoTA open-set semi-supervised classification method. We experiment on COCO-open with $4k$ images from 20 selected ID objects.}
\label{table:coco-openmatch}
\vspace{-4mm}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{ccccc}
\toprule
Method & Label-only & UT    & OpenMatch & Ours (UT+DINO) \\ \midrule
mAP                 & 17.60      & 18.95 & \underline{20.06}     & \textbf{24.01}     \\
% $\Delta$            & -      &  \textcolor{myblue}{+1.35} & \textcolor{myblue}{+2.46}     & \textbf{\textcolor{myblue}{+6.41}}  \\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}




==> table/rebuttal/os_object.tex <==
\begin{table}[h]
\centering
\vspace{-2mm}
\renewcommand{\arraystretch}{1.3}
\caption{Adaptation of the open-set object detection work, ORE (Joseph et al., \href{https://arxiv.org/abs/2103.02603}{CVPR'21}), to our OSSOD setting (COCO-open with 4k images from 20 ID objects). }
\label{table:coco-ore}
\vspace{-4mm}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{ccccc}
\toprule
Method    & Label-only & UT     & ORE  & \textbf{Ours}\\ \midrule
mAP       &   17.60    & 18.95  &   \underline{21.55}   & \textbf{24.01}  \\
% $\Delta$            & -      &  \textcolor{myblue}{+1.35} & \textcolor{myblue}{+2.46}     & \textbf{\textcolor{myblue}{+6.41}}  \\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}


==> table/rebuttal/ossod.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
Comparison to SSOD methods in COCO-additional.
}
\vspace{-3mm}
\label{table:rebut_cocoadd_sota}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{cc}
\toprule
& mAP   \\ 
\midrule
% CSD (NeurIPS'19)                        & 38.82 \\
Instant-Teaching (CVPR'21)              & 40.20 \\
Humble Teacher (CVPR'21)                & 42.37 \\
Unbiased Teacher* (ICLR'21)             & 44.06 \\
SoftTeacher (ICCV'21)                   & 44.05 \\
Ours                                    & \textbf{45.14} \\ 
\bottomrule
\end{tabular}
}
\vspace{-7mm}
\end{table}


==> table/rebuttal/softteacher.tex <==
\begin{table}[h]
\centering
\vspace{-3mm}
\renewcommand{\arraystretch}{1.3}
\caption{Integration our method with SoftTeacher (Xu et al., \href{https://arxiv.org/abs/2106.09018}{ICCV'21})), the SoTA SSOD method. We experiment on COCO-open with $4k$ images from 20 ID objects (20/60). 
The result for SoftTeacher below is from single run.
% \kevin{Where does 24.01 from UT came from? The number is different from Table 2 in the original paper}\yc{Here is single run, and Table 2 is averaged over multiple runs. Should we use mean of Table 2 ? }
}
\vspace{-4mm}
\label{table:coco-open-softteacher}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
Method &   UT     & SoftTeacher \\ \midrule
Original    &       18.37 &  19.46            \\
\textbf{Ours (offline DINO)}    &        \textbf{23.43} \scriptsize{\textcolor{myblue}{(+5.06)}} &  \textbf{24.91} \scriptsize{\textcolor{myblue}{(+5.45)}}            \\

% $\Delta$            & -      &  \textcolor{myblue}{+1.35} & \textcolor{myblue}{+2.46}     & \textbf{\textcolor{myblue}{+6.41}}  \\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}


==> table/rebuttal/ssod.tex <==
\begin{table}[h]
\centering
\vspace{-3mm}
\renewcommand{\arraystretch}{1.3}
\caption{Adapting our method to the closed-set SSOD does not hurt the results, and we instead improve UT (Liu \textit{et al.}, \href{https://arxiv.org/abs/2102.09480}{ICLR'21}).}
\label{table:coco-closed}
\vspace{-4mm}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
Experiment & Method & Label-only & UT     & \textbf{Ours (UT+DINO)}  \\ \midrule
COCO-standard $1\%$ & mAP      & 9.34      &  20.69 &  \textbf{21.08}  \\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}


==> table/stat_coco_open.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{The statics of COCO-Open.}
\vspace{1mm}
\label{table:ap_breakdown_all}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
                         & \multicolumn{5}{c}{COCO}                               \\\cmidrule{2-6}
No. of Known/Unknown     & \multicolumn{2}{c}{40/40} & & \multicolumn{2}{c}{60/20} \\ \cmidrule{2-3} \cmidrule{5-6}
No. of Labeled Data      & 1,000        & 4,000    &   & 1,000        & 4,000       \\         \specialrule{1pt}{1pt}{1pt}
Labeled only             & 10.94        & 16.07     &  & 10.46        & 17.32       \\ \
UT~\cite{liu2021unbiased}         & 15.47        & 19.93  &     & 16.84        & 22.83       \\ \midrule 
UT~\cite{liu2021unbiased} + OoD (DINO)  & 17.22        & 23.31  &     & 18.02        & 25.42       \\ 
UT~\cite{liu2021unbiased} + OoD (ViT-B) & 19.63        & 25.32  &     & 19.67        & 26.17       \\ 
\bottomrule
\end{tabular}
}
% \vspace{-3mm}
\end{table}

